Nudge: Accelerating Overdue Pull Requests Towards Completion

Pull requests are a key part of the collaborative software development and code review process today. However, pull requests can also slow down the software development process when the reviewer(s) or the author do not actively engage with the pull request. In this work, we design an end-to-end service, Nudge, for accelerating overdue pull requests towards completion by reminding the author or the reviewer(s) to engage with their overdue pull requests. First, we use models based on effort estimation and machine learning to predict the completion time for a given pull request. Second, we use activity detection to filter out pull requests that may be overdue, but for which sufficient action is taking place nonetheless. Lastly, we use actor identification to understand who the blocker of the pull request is and nudge the appropriate actor (author or reviewer(s)). The key novelty of Nudge is that it succeeds in reducing pull request resolution time, while ensuring that developers perceive the notifications sent as useful, at the scale of thousands of repositories. In a randomized trial on 147 repositories in use at Microsoft, Nudge was able to reduce pull request resolution time by 60% for 8,500 pull requests, when compared to overdue pull requests for which Nudge did not send a notification. Furthermore, developers receiving Nudge notifications resolved 73% of these notifications as positive. We observed similar results when scaling up the deployment of Nudge to 8,000 repositories at Microsoft, for which Nudge sent 210,000 notifications during a full year. This demonstrates Nudge's ability to scale to thousands of repositories. Lastly, our qualitative analysis of a selection of Nudge notifications indicates areas for future research, such as taking dependencies among pull requests and developer availability into account.

==> Implementation.tex <==
\section{Implementation} \label{Implementation}

\begin{figure*}
\includegraphics[width=\textwidth]{figures/workflow.png}
\vspace{-1.5\baselineskip}
\caption{Architecture of the PRLifetime Service}
\label{fig:architecture}
\end{figure*}

\label{sec:examples}
In this section we discuss the implementation details for the PRLifetime Service. We start by discussing Azure DevOps on which it is deployed as an extension. Further, we describe the various components of the PRLifetime Service: 1) Data pipeline 2) Model Training 3) Inference 4) Notification. Figure \ref{fig:architecture} shows a high level overview of the service architecture.

\subsection{Azure DevOps} 

Azure DevOps (ADO) is a DevOps platform providing GIT based VCS (version control system) along with collaboration tools for developers such as Pull Request based code reviews, work item tracking and, also, planning tools for sprints / scrums. Lastly, it also enables CI / CD of code through CD pipelines. ADO is heavily used across Microsoft internally for product development. We have built and deployed PRLifetime Service as an extension of ADO because of the rich collaboration features. We also used ADO repository for developing the PRLifetime Service, allowing us to dogfood the feature within our own team as well. Below we talk about two main aspects of ADO which were crucial for the PRLifetime service: 
\begin{enumerate}
    \item \textbf{Code Reviews} - ADO provides a rich set of features for doing code reviews for the code in the ADO repositories. To push any changes to the master branch of a repository, developers create Pull Requests (PR) and request their team members to review and approve the PRs. The reviewer can then either a) approve the PR or b) add inline comments on the PR and ask the PR author to revise the PR. The comments posted in the PR are visible to all the participants of the PR i.e. author and reviewers. As shown later in Figure \ref{fig:screenshot}, we leverage this comment functionality and add a comment whenever a PR has been pending for a significant time. We further discuss this in detail in Section 2.2. 
    \item \textbf{APIs} - ADO exposes a rich set of REST APIs ~\cite{AzureDevOpsRest} to enable extensibility. These APIs not only allow us to ingest data from ADO for various entities such as Commits, Work Items, Pull Requests but also allows us to interact with the PR by adding comments, reviewers etc.
\end{enumerate}

\subsection{Nudge Service Implementation} 
The Nudge service is implemented using C\# and .NET 4.6. It's built on top of Microsoft Azure Cloud Services using Azure Batch ~\cite{AzureBatch} for compute, Azure SQL for data storage, Azure Active Directory for authentication and Application Insights for telemetry and alerting. We used ADO for collaborative development of the services and, also CI / CD for the codebase. To enable the service on an ADO repository, the ADO project admin grants access to the repository to a system account. Subsequently, the data pipelines in the PRLifetime Service start ingesting the data for training models and starts interacting with the PRs. The major components of the services are: \\
\textbf{Backend Pipeline} - We leverage Azure Batch for scaling the PRLifetime Service data pipelines which are responsible for data ingestion and, also decorating the PRs with comments. Azure Batch is a PaaS service for building high performance and parallel applications and abstracts out critical components such as the job scheduler, the compute resource provider, etc. Azure Batch allows us to scale horizontally as more and more repositories are onboarded. We create a job schedule for each of the onboarded repository and a job is triggered every 6 hours. As we onboard more repositories, our deployment auto scale the compute resources. 
A Batch job basically ingests/updates any new entities (PRs, Commits, etc.) using the ADO APIs that have been created or updated since the last run. Further, it also does inference and decoration of PRs. 
\\
\textbf{Data Store} - We use SQL Azure for storing the data and features used by the PRLifetime Service. We have a normalized schema for representing various entities like PRs, Commits, Users, etc. For each repository we onboard, we create a separate database. We use the Elastic Pool feature in SQL Azure to minimize the resource requirements. This allows us to be very efficient in terms of per repository cost. 
\\
\textbf{Training data} - We train our machine learning models using a subset of the PRs ingested. Based on our manual analysis, to reduce the noise, we exclude two sets of PRs: 
\begin{enumerate}
    \item PRs with completion times less than 24 hours. We observed that if a PR is completed in few hours or within a day, most likely it is a  change that needs to be rolled out immediately; like a security fix or some critical bug fix. In that case the PR is reviewed and merged on an accelerated schedule.
    \item PRs with completion time greater than 2 weeks. If a PR is sitting in the system for more than two weeks, as per our observation, they are mostly draft PRs or PRs that were abandoned due to a decision taken offline or PRs which are not that important but created and left around by the author before they head to a vacation or taking a time off. 
\end{enumerate}
\textbf{PRs used for training} = All the completed PRs - (PRs with less than 24 hours of lifetime + PRs with more than two weeks of lifetime)

\textbf{Inference} - For the ML predictions, we have trained and deployed the model in a Flask based python service in Azure. When the backend pipeline runs, it takes all the PRs that are active and have spent at least 24 hours in the system (this filter is due to the reasons mentioned in the model training section above). Then, we extract all the features in our feature space, for the current PR, and create a feature vector. Once the feature vectors are created for all the PRs for which we are planning to do inference, we make REST calls to the inference API we already deployed. Inference results for each PR (predicted Lifetime) is then saved in our cloud database.
\\
\textbf{Notification to the Developers} During every run of our pipeline, we look at all the PRs that meet all of the following criteria:
\begin{enumerate}
    \item PRs that are active. 
    \item PRs for which predicted lifetime is generated and saved in our database, during the previous run of the pipeline.
    \item PRs for which we have not already generated a notification earlier
    \item Age of the PR is at least (predicted lifetime + 24 hours).
\end{enumerate}
We consider such PRs as a candidate for notification and a notification is sent to the PR author and reviewers of the PR to act on it (as shown in Figure \ref{fig:screenshot}). Time of notification (Tn) is defined as:
\[ Tn = Tc + Tp + \mbox{24 hours} \]    
where Tc is the PR creation date time and Tp is the predicted lifetime for a PR (in hours).
After doing user studies and talking to various developers and managers, we decided to give a buffer time of 24 hours to account for variations in work schedules.

\subsection{Activity detection} We use \ado{}'s REST APIs[cite] extensively to collect data that is required to understand if there has been any activity in a \pr{}. We gather data about various actions or activities that happen inside a \pr{} (as explained in section \ref{ActivityDetection}) to determine if there has been any activity.

\begin{itemize}
    \item \textbf{Commit activity} We use \ado{}'s GetPullRequestIterationsAsync API which provides details about all the commits that are ever pushed into a \pr{}. We first get a list of all the commits that are pushed using the GetPullRequestIterationsAsync API then take the timestamp of the latest iteration as the latest commit timestamp of a \pr{}.
    \item \textbf{Comment activity} To determine whether there has been any commenting activity like adding new comments or replying to existing comments, we use \ado{}'s GetThreadsAsync API. This API returns all the comments that are ever placed in a \pr{} in the form of threads. We check if any new threads are created or any new comments are placed in an existing thread. We take the maximum of both of them to determine the latest comment activity that has happened in a \pr{}. While doing this we exclude any comments that are placed by system accounts or non-human actors.
    \item \textbf{State changes in \pr{}s} Changes in \pr{} state is another important signal that helps determining activity in a given \pr{}. Unfortunately, there is no direct way of determining state changes in \pr{}s. We use \ado{}'s GetThreadsAsync API to collect all the comments placed in a \pr{}. Comments whose content property contains the word "voted" indicates that a state change has happened. We use that to determine when was the last time time a \pr{}'s state has changed.
\end{itemize}


\subsection{Dependency determination} We rely heavily on \ado{}'s REST APIs again to collect data that is required to determine dependencies. As explained in section \ref{DependecyDetermination}, we need to understand the three primary constructs listed below to determine dependencies.

\begin{itemize}
    \item \textbf{Is \pr{} waiting on the Author?} To determine if \pr{}'s author has any pending action items, we check if the state of the \pr{} is set to 'Waiting on Author'. We use \ado{}'s GetPullRequestReviewersAsync API to get the votes of all the reviewers. We check if there are any votes with status "-5" which indicates that the \pr{} is marked as 'Waiting on author' by one of the reviewers.
    \item \textbf{Check for existence of unresolved comments} Understanding the existence of unresolved comments is important to understand if the blocker of the \pr{} is the author or the reviewer. We use \ado{}'s GetThreadsAsync API to get all the threads and then we check for existence of threads with statuses 'Active' or 'Pending'. Presence of threads with any of these two statues indicates that there are unresolved comments 
    \item \textbf{Enumerate the list of change blockers} We first use GetPullRequestReviewersAsync API offered by \ado{} to query the list of reviewers on a given \pr{}. We then use GetThreadsAsync API to determine list of all the reviewers who commented on the \pr{} at least once and who comments are resolved by the author of the \pr{}. We prepare two lists: commented reviewers and all reviewers and choose one of them to use based on the state of the \pr{}. If there are no reviews on a \pr{}, we send notifications to the reviewers in the 'all reviewers' list. If there has been review activity (placing comments on the \pr{} by a reviewer), we prioritize notifications to the reviewers in the commented reviewers list.
\end{itemize}

Figure \ref{fig:Screenshot} shows screenshot of how the notification looks like with the enhanced versions of the service. In the enhanced version the dependant actors (in this case the reviewer but not the author) is '@ mentioned'. This triggers a separate email addressing to the reviewer of this \pr{} is sent requesting them to unblock the \pr{}. As we can notice, The \pr{} was created and had been waiting for the reviewer's approval for four days. After the \PaperTitle\ service tagged the reviewer and pushed them to act on the \pr{}, the reviewer has approved it and the \pr{} got completed on the same day.

 



==> Results.tex <==
\section{ Results }
\label{sec:eval}

We would like to answer two important questions here when we talk about results. 
\begin{enumerate}
    \item How accurate is a prediction/estimate? 
    \item Are we helpful in driving a PR towards a terminal state {'Completed' or 'Abandoned'}? If so, by what margin are we expediting? 
\end{enumerate}
To answer question 1, we generated metrics and visualizations that explain how accurate our prediction model is (we will be taking about in section 4.2). And, to answer question 2, we generated metrics to capture quantitative feedback and interviewed the developers on whose PRs we made suggestions and gathered qualitative feedback. 
In the subsequent sections, we are going to discuss both our quantitative and qualitative analysis.

\subsection{Model Evaluation}

\begin{figure}
\includegraphics[width=\columnwidth]{figures/mae.png}
\vspace{-1.5\baselineskip}
\caption{MAE distribution}
\label{fig:mae}
\end{figure}

We evaluated our prediction model against standard metrics: MAE and MRE. The Mean Absolute Error (MAE) is 32.60 hours and Mean Relative Error (MRE) is 0.58. To put these numbers in perspective, we have done an experiment by considering mean lifetime of our training data as the predicted lifetime of every PR in our testing data. Our random model's MAE is 36.43 hours and MRE is turned out to be 0.68. We are doing 11.8\% better with MAE and 17.7\% better with MRE compared to the random model. 
To understand if a MAE of 32.60 hours is reasonable, we should also understand few important metrics of the data on which we are training and doing inference against. The data set we are dealing with has a mean PR Lifetime of 107.63 hours and the earliest a PR is completed is in 24 hours (minimum) \& a maximum lifetime of a PR is 336 hours. Basically, we have a prediction MAE of 32.60 for data points (PRs) ranging from 24 hours to 336 hours. Figure \ref{fig:mae} shows the MAE distribution. A very interesting thing to note is, a significant portion of our MAE lies within the range of 50 hours and only a very little portion of our absolute error exceeds order of 107 hours (which is the mean of this distribution).

\begin{figure}[b]
\includegraphics[width=\columnwidth]{figures/mre.png}
\vspace{-1.5\baselineskip}
\caption{MRE distribution}
\label{fig:mre}
\end{figure}

An important thing to note is, majority of our MRE (close to 90\%) falls under a relative error of 1. Figure \ref{fig:mre} shows the MRE distribution. As with any regression problems, one of the other important metrics to understand is tolerance. Based on the domain we are operating in and the users who are consuming our prediction results, tolerance levels may vary. For instance, in real estate or in finance, a tolerance of 50\% is not acceptable. However, in effort estimation, going off by +/- 50\% hours is reasonable since we are only notifying developers for acting on pending Pull Requests. In our Qualitative analysis section (4.3), we list anecdotes from users which supports this argument. The distribution of our prediction accuracy based on the tolerance level is listed in Table \ref{tolerance}.

\begin{table}
\caption{Tolerance level distribution}
 \begin{tabularx}{\columnwidth}{|X|X|} 
 \hline
 Tolerance level & \% of predictions within tolerance level \\
 \hline
 +/- 0\% & 0.7 \\
 \hline
+/- 5\% & 7.17 \\
 \hline
+/- 10\% & 13.97 \\
 \hline
+/- 15\% & 21.33 \\
 \hline
+/- 20\% & 28.44 \\
 \hline
+/- 30\% & 41.06 \\
 \hline
+/- 50\% & 62.91 \\
 \hline
+/- 70\% & 74.44 \\
 \hline
+/- 90\% & 79.82 \\
 \hline
+/- 100\% & 81.29 \\
 \hline
\end{tabularx}
\label{tolerance}
\end{table}

\subsection{Quantitative Analysis}
 
For every comment (as shown in Figure 3) we add in every PR, we calculate comment resolution percentage (CRP). CRP indicates how many comments made by us are honored and/or agreed on by the author of the PR.
\[\mbox{CRP = No. of comments resolved / Total no. of comments made}\]
We looked at the comments added by our system in all the 43 repositories in which it is enabled. We have made 1069 comments in last three months and our comment resolution percentage is 73.3. To descriptively put, 73 out of 100 comments made by us are resolved by the developers and indicate that developers agree with our recommendations. We realized that while CRP indicates a strong agreement by the author, we did another analysis (explained below) to understand if the PRs are getting completed faster because of the comments we are adding.
\par To assess the empirical efficacy of the comments, we compare the PR completion times for notified PRs and non-notified PRs (shown in Table \ref{average-completion-time}). As described in Section 2.2, we notify PR authors for PRs which are 24 hours past the predicted PR completion time. In total, we notified the author of 913 PRs which are over 24 hours past the predicted PR time. We found that after decorating the PR completion time on average is 115.81 hours after the PR decoration. To compare against the scenario where we have no PR decoration, we look at 5769 older PRs. For these PRs we split the time as predicted+24 hours in one bucket and the time remaining after subtracting the predicted+24 hours. The Average time in this case is 165.54 hours. Comparing this with the 115.81, conservatively we see a quicker turnaround to resolving and closing PRs by 43\%. 
Additionally, we observe that most PRs are completed within a week of decoration without comment. The distribution of the completion times of the PRs after the decoration is shown in Figure \ref{fig:prcompletion-times}.


\begin{figure}
\includegraphics[width=\columnwidth]{figures/prcompletion-times.png}
\vspace{-1.5\baselineskip}
\caption{Distribution of PR completion times after decoration}
\label{fig:prcompletion-times}
\end{figure}



\begin{table}[b]
\setlength\belowcaptionskip{7pt}
 \caption{Average PR completion time comparison}
 \begin{tabularx}{\columnwidth}{|X|X|X|} 
 \hline
 Category & Count & Time from decoration to completion (AVG) \\
 \hline
 Non-Notified PRs & 5769 & 165.54 \\
 \hline
 Notified PRs & 913 & 115.81 \\  
 \hline
\end{tabularx}
\label{average-completion-time}
\end{table}

\begin{figure*}
\includegraphics[width=\textwidth]{figures/Comment-Screenshot.PNG}
\vspace{-1.5\baselineskip}
\caption{Nudge notification on a Pull Request}
\label{fig:screenshot}
\end{figure*}

\subsection{Developer Feedback}
In addition to quantitative analysis, we have reached out to developers from various product groups (17 people, including managers) on whose PRs we added a comment. We interviewed them and tried to understand what they think about our service. To paraphrase, our evaluation metrics are checking two things essentially: 1). If the comment we are adding in their PR is helping them drive the PR towards completion 2). If the number of hours we are predicting as the estimated lifetime of a PR are making sense. We decided not to make the interview anonymous and pinged people directly on Skype/Teams. We did not make an effort to make it anonymous because, the quality of responses is not going to be impacted as we are not asking any personal questions that make people frank and honest about their responses in an anonymous setting. In this interview, we asked two open-ended questions: 
\begin{enumerate}
    \item If this comment has any value add? Do you think it helps you moving / acting on this PR towards completion or abandonment?
    \item Do you think the predicted PR completion time is reasonable?
\end{enumerate}

\subsubsection{Helpfulness in driving PRs towards completion / abandonment}
We tried to understand how helpful our suggestions are and whether they are yielding intended benefits i.e., driving PRs towards a terminal state which is Completion or Abandonment.  We received very positive feedback (comments/anecdotes from the developer) and observed that intended actions are happening on the PRs. On one of the PRs, a developer said 
\textit{"I agree. Making few more changes and pushing this PR through! Thanks!"}
Then we saw this developer acting on this PR by pinging the reviewers and driving this PR towards completion. And within 8 minutes this PR got completed. In another PR, the developer has acknowledged our nudge and completed it within a day. 
In another PR, the developer has done something very interesting. First, he replied to our comment saying  
\textit{"The pipeline is failing and blocking this check in. Followed up with an ICM incident!"} 
then, soon enough (within a day) the PR was abandoned. Here, it is not just about completion, people are making progress on their PRs by pushing them towards a terminal state (completion/abandonment) and in turn maintaining the repository hygiene. So, we are clearly seeing that people are responding to the comments and most importantly, taking an action to push the PRs towards completion/abandonment thus expediting the deployment of changes and achieving repository hygiene. There are few situations where we received feedback that says the comment that we made and the attempt to capture developer's attention to drive their PRs towards completion is not very helpful. A comment from one of our interview respondents is  
\textit{"The comment does not add any value to me personally because 1) I already know that the PR I've authored / am reviewing has been open for a long time, 2) I am currently working on doing better at looking at PRs earlier, so basically all the PRs I've reviewing have this, 3) I have the emails about PRs that come to my inbox highly filtered to cut down on noise, so I only see these comments when I'm on the PR already"} 
As the developer above has mentioned, sometimes a PR is set to wait due to few external factors like, dependency on other \pr{}s or management decisions like feature planning and road-maps etc. In these cases, pinging the developer and re-iterating the fact that their PR is safe to complete (especially when they are staying on top of that PR) doesn't seems to be adding much value. As part of our future work, we are planning to come up with a way to systematically determine the external factors that are blocking a PR  and nudge the right people but not the authors of the PR (especially if they do not have any action item pending on their side or can't do anything to move their PR forward). 

\subsubsection{Accuracy of predictions for Pull Request completion time}
We tried to understand how accurate our estimation is for PRs' completion time and we presented various metrics that bolster our accuracy claims in the quantitative analysis section. Here we are listing few anecdotes from the developer/author of the PR. 
\textit{"Yes, I thought the approximation was pretty good"}
Another developer, from a different PR and different repository says 
\textit{"The approximation does sound about right. I went on-call which led to delay in check-in in this case. Normally, it would have been within about that range"}


 




==> reference.tex <==
% \section{References}
% \begin{itemize}
%     \item KDD,Post-processing of association rules 
% \end{itemize}

\nocite{*}
\bibliography{paper}
\bibliographystyle{abbrv}

%Auto-fixing misconfiguration:
%https://ieeexplore.ieee.org/abstract/document/8115673

%https://www.ics.uci.edu/~andre/ics228s2006/zimmermanweissgerberdiehlzeller.pdf
%	https://www.microsoft.com/en-us/research/wp-content/uploads/2016/02/barnett2015hdh.pdf
%	https://www.cs.mcgill.ca/~martin/papers/esecfse2005a.pdf
%	https://ieeexplore.ieee.org/document/5770624
%	https://ieeexplore.ieee.org/document/6606615

%correlated configuration: https://tianyin.github.io/papers/asplos14.pdf
%Configuration is complex: https://tianyin.github.io/papers/fse15.pdf  
%Early detection: https://www.usenix.org/conference/osdi16/technical-sessions/presentation/xu
%Facebooks config management: https://research.fb.com/wp-content/uploads/2016/11/holistic-configuration-management-at-facebook.pdf
% strider, peer pressure
%correlated configuration: https://tianyin.github.io/papers/asplos14.pdf
%Configuration is complex: https://tianyin.github.io/papers/fse15.pdf  
%Early detection: https://www.usenix.org/conference/osdi16/technical-sessions/presentation/xu
%Facebooks config management: https://research.fb.com/wp-content/uploads/2016/11/holistic-configuration-management-at-facebook.pdf
% strider: https://www.sciencedirect.com/science/article/pii/S0167642304000760
% peerpressure https://www.usenix.org/legacy/publications/library/proceedings/osdi04/tech/full_papers/wang/wang.pdf





% https://www.cs.sfu.ca/~jpei/publications/sigmod00.pdf
% http://www.cse.msu.edu/~cse960/Papers/MiningAssoc-AgrawalAS-VLDB94.pdf
% http://www.cs.tau.ac.il/~fiat/dmsem03/Efficiently%20mining%20long%20patterns%20from%20databases%20-%201998.pdf
% http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.41.6476&rep=rep1&type=pdf


%xmldiffpatch : https://www.nuget.org/packages/XMLDiffPatch/
% roslyn : https://github.com/dotnet/roslyn
%getafix: https://arxiv.org/pdf/1902.06111.pdf

%anti-unification : https://core.ac.uk/download/pdf/62916252.pdf




